Top-Personalized-K Recommendation

The conventional top-K recommendation, which presents the top-K items with the highest ranking scores, is a common practice for generating personalized ranking lists. However, is this fixed-size top-K recommendation the optimal approach for every user's satisfaction? Not necessarily. We point out that providing fixed-size recommendations without taking into account user utility can be suboptimal, as it may unavoidably include irrelevant items or limit the exposure to relevant ones. To address this issue, we introduce Top-Personalized-K Recommendation, a new recommendation task aimed at generating a personalized-sized ranking list to maximize individual user satisfaction. As a solution to the proposed task, we develop a model-agnostic framework named PerK. PerK estimates the expected user utility by leveraging calibrated interaction probabilities, subsequently selecting the recommendation size that maximizes this expected utility. Through extensive experiments on real-world datasets, we demonstrate the superiority of PerK in Top-Personalized-K recommendation task. We expect that Top-Personalized-K recommendation has the potential to offer enhanced solutions for various real-world recommendation scenarios, based on its great compatibility with existing models.

==> 1Intro.tex <==
\begin{figure}[t]
\begin{subfigure}[t]{0.99\linewidth}
    %\includegraphics[width=\linewidth]{figure/intro.png}
    \includegraphics[width=\linewidth]{figure/intro_double.png}
\end{subfigure}
\vspace{-0.2cm}
%\caption{An example of top-$K$ recommendation with a fixed size of five and top-personalized-$K$ recommendation. 1 and 0 represent the relevant and the irrelevant item, respectively. Note that these labels are not available at the inference phase.}
\caption{An example of top-personalized-$K$ recommendation. 1 and 0 represent the relevant and the irrelevant items, respectively. Note that these labels are not available at the inference phase. Newly added items have red outlines.} %  
%\vspace{-0.cm}
\setlength{\belowcaptionskip}{-10pt}
\setlength{\abovecaptionskip}{-5pt}
\vspace{-0.7cm}
\end{figure}

Personalized recommendations have a significant impact on various daily activities such as shopping, advertising, watching videos, and listening to music.
To generate personalized ranking lists of items, recommender systems utilize the top-$K$ recommendation approach \cite{topk10}, which presents the $K$ items with the highest ranking scores, sorted in descending order.
This approach has become a common practice in recent recommender systems \cite{sgl21, topk22, topkk22} due to its optimality with the globally fixed recommendation size \cite{prp77}.
However, while tremendous efforts have been made on recommender models, an important question has been overlooked in the previous literature: \textit{is the fixed-size top-$K$ recommendation the optimal approach for ensuring every user’s satisfaction?} %for the top-$K$ recommendation

To elucidate the potential drawbacks of the top-$K$ recommendation approach, we start with a motivating example in Figure 1.
%With the top-$K$ recommendation, user 1 is presented with two irrelevant items in the tail.
%In this case, the top-$K$ recommendation \textit{unavoidably includes} irrelevant items as the ranking list is not filled with enough relevant items.
For user 1, the top-$K$ recommendation \textit{unavoidably includes} two irrelevant items in the tail, as the ranking list could not be filled with enough relevant items.
%However, irrelevant items are not only useless but even harmful \cite{sigir22}.
%Exposure to irrelevant items could result in user dissatisfaction and lead to users ignoring future recommendations (i.e., ad blindness) \cite{swing08} or leaving the system \cite{leave06}.
However, exposure to irrelevant items could result in user dissatisfaction and lead to users ignoring future recommendations (i.e., ad blindness) \cite{swing08} or leaving the system \cite{leave06}.
On the other hand, user 2 receives a more accurate top-$K$ recommendation with four relevant items.
However, the recommendation could also be further improved by including one additional relevant item in the tail.
Limited exposure to relevant items can curtail user engagement, potentially leading to a decline in revenue \cite{revenue19}.
This example shows that the top-$K$ recommendation with a globally fixed recommendation size cannot ensure optimal user satisfaction.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% Moreover, fixed recommendation size may further degrade the efficiency of real-world systems with constrained resources (i.e., presenting the same number of items ) 
%Furthermore, drawbacks induced from fixed size can be exaggerated, when it comes to real-world applications like presenting the same number of items from each domain without consideration of the user's preference in Figure 1.
Moreover, as illustrated in Figure 1 bottom, limitations arising from the fixed size scheme can be exacerbated in real-world scenarios, such as presenting an equal number of items from each domain without considering user preferences.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this sense, we claim that the recommendation size needs to be engineered alongside the recommender model.

In this work, we propose \textbf{Top-Personalized-$K$ Recommendation}, a new recommendation task resolving the limitation of the top-$K$ recommendation.
Formally, the top-personalized-$K$ recommendation refers to providing a ranking list of the personalized size that maximizes individual user satisfaction, which can be quantitatively measured by user utility \cite{fair18, saito22fair}.
Back in Figure 1, the top-personalized-$K$ recommendation can increase both users' satisfaction by reducing the effort spent inspecting irrelevant items (user 1) and providing more relevant items (user 2). %% 앞 문단 수정에 맞게 바꾸기
% Furthermore, while our work primarily focuses on the technical facets, the proposed task has several implications for real-world applications and research:
Furthermore, the proposed task has several implications for real-world applications, especially for systems with limited resources for making recommendations: % while our work primarily focuses on the technical facets, 
(1) \textit{Multi-domain recommender systems} \cite{cdr12} that display items from various domains on a single constrained screen can strike a balance in recommendation sizes by employing adapted-sized ranking lists from each domain (Figure 1 bottom). % balance라는 말이 맞나?
(2) In the case of \textit{sponsored advertisements} \cite{swing08}, advertisers can achieve higher user engagement with the same promotion expenses by adjusting the number of promoted items based on each user's expected utility.
(3) In the context of the \textit{prefetching mechanism} \cite{prefetch16}, which caches the initial few seconds of videos expected to be clicked in order to reduce startup delay, the system can minimize cache size and prevent cache pollution by adjusting the number of items to be cached. % 

We propose a novel framework named \textbf{PerK}, as a solution to the top-personalized-$K$ recommendation task.
PerK is agnostic to the model architecture, allowing it to be adapted for any item recommendation scenario with existing recommenders.
We first formulate a bi-level optimization problem where the objective is to determine the recommendation size that maximizes the user utility (Sec 4).
To solve this optimization, we need to acquire the user utility for each candidate size.
However, it is not feasible to directly compute the user utility, since we do not have access to the true relevance of unobserved items. % in the ranking list.
To address this problem, we introduce the concept of \textit{expected user utility} and estimate it instead of its true value (Sec 5.2).
%We treat the interaction labels of unobserved items as Bernoulli random variables and estimate the expectation of the user utility with respect to those random variables.
%Based on this modeling, we derive computational forms of the expected user utility for various widely-used utility measures.
We treat the interaction labels of unobserved items as Bernoulli random variables and derive the expectation of the user utility for various widely-used utility measures. %  with respect to those random variables.
%Based on this modeling, we derive computational forms of the expected user utility for various widely-used utility measures.
Derived expected user utilities can be computed with the interaction probability of user-item pairs.
% and allow us to select the recommendation size with the maximum expected user utility.

The remaining challenge is obtaining accurate interaction probability with an arbitrary recommender model.
The recommender models do not necessarily output the accurate interaction probability \cite{cal17, kweon22}.
They often output unbounded ranking scores that cannot be treated as probabilities \cite{bpr09, lightgcn20} or miscalibrated interaction probabilities that do not accurately reflect the true likelihood of user-item interactions \cite{ncf17,vae18}.
To address this problem, we propose the use of \textit{calibrated interaction probability} obtained through the user-wise calibration function (Sec 5.3).
The calibration function maps the ranking scores of the recommender model to well-calibrated interaction probabilities \cite{kweon22}.
We adopt Platt scaling \cite{platt99} and instantiate it for each user to consider the different distributions of the ranking score across users. % , a simple and widely-adopted calibration function,
We train the calibration function to predict the interactions between pairs in a held-out calibration set. % held out for each user.
As a result, the output of the function accurately indicates the true likelihood of interaction, leading to accurate expected user utility.

In summary, we aim to find the optimal recommendation size for each user by (1) obtaining calibrated interaction probability with user-wise calibration, (2) estimating the expected user utility, and (3) determining the recommendation size that results in the maximum expected user utility.
The main contributions of our work can be described as follows:
\begin{itemize}[leftmargin=*]
    \item We highlight the necessity of personalized recommendation size based on its practical advantages in real-world scenarios, which has not been studied well in the previous literature.
    \item We propose Top-Personalized-$K$ Recommendation, a new recommendation task where the recommendation size can be adjusted for each user to enhance individual user satisfaction.    
    \item We develop PerK, a framework to determine the personalized recommendation size by estimating the user's expected utility with the calibrated interaction probability.
    \item We conduct comprehensive experiments with three base recommenders on four real-world datasets, demonstrating the superiority of PerK in the top-personalized-$K$ recommendation task.
\end{itemize}






\begin{comment}
However, a globally fixed $K$ value for top-$K$ recommendation may not be optimal for maximizing user utility.
The optimal $K$ that maximizes user utility may vary for each individual user based on the accuracy of the recommendations.
If the recommendation is accurate, it would be beneficial for the system to present all confident items in order to increase user utility.
On the other hand, presenting too many irrelevant items could result in user dissatisfaction and even lead to users leaving the system \cite{leave06}.
The recommendation size serves as a key factor in striking a balance between these two situations.
Therefore, we claim that the recommendation size is also a fundamental component affecting user utility and needs to be engineered alongside the recommender model itself.
Despite its importance, the methodology for determining the appropriate number of items to recommend has received surprisingly little attention in the literature.

In this work, we propose \textbf{Top-Personalized-$K$ Recommendation}, a novel framework for finding a personalized $K$ value for the top-$K$ recommendation.
In our framework, the recommendation size is treated as a variable rather than globally fixed.
We formalize a bi-level optimization for our framework and determine the optimal recommendation size by selecting the one that results in maximum user utility.
However, it is not feasible to directly compute the user utility since we do not have access to the interaction label for unobserved items.
To address this, we introduce the concept of \textit{expected user utility} and estimate it instead of its true value.
We develop mathematical models for estimating the expectation of the user utility with respect to the random variables that represent the user-item interactions.
Based on this model, we derive computational forms of the expected user utility for various widely-used utility functions.
These formulations can be computed with the probability of interaction between user-item pairs, thus allowing us to select the recommendation size with the highest expected user utility.

\begin{itemize}[leftmargin=*]
    \item We address the necessity of personalized recommendation size for the top-K recommendation to improve user utility, and propose the Top-Personalized-$K$ Recommendation framework to optimize $K$ values for individual users.
    \item We develop mathematical models for estimating the expected user utility and introduce a user-wise calibration function to obtain accurate interaction probabilities with arbitrary recommenders.
    \item We conduct a comprehensive experiment with three recommenders on four real-world datasets, and demonstrate that the proposed framework provides personalized $K$ values for each user that result in higher user utility compared to competitors.
\end{itemize}
\end{comment}

==> 6EX.tex <==
\subsection{Experiment Setup}
%We validate the superiority of the proposed task (Top-Personalized-$K$ Recommendation) and the proposed framework (PerK) through extensive experiments on 4 real-world datasets × 3 base recommender models × 4 utility measures. % 줄이기 가능
%Please refer to Appendix A.2 for a detailed experiment setup.
We provide a summary of the experiment setup due to limited space.
Please refer to Appendix A.2 for more details.
We will publicly provide the GitHub repository of this work in the final version.

\subsubsection{Datasets}
%\noindent \textbf{Datasets.}
We use four real-world datasets including MovieLens 10M,\footnote{https://grouplens.org/datasets/movielens/} CiteULike \cite{citeulike13}, MovieLens 25M, and Amazon Books \cite{amazon19}.
These datasets are publicly available and have been widely used in the literature \cite{ncf17, lightgcn20, cdl15, cvae17}.
%We adopt the 20-core setting for all datasets as done in MovieLens datasets.
%Data statistics after the preprocessing are presented in Table 1.
We randomly split each user’s interactions into a training set (60\%), a validation set (20\%), and a test set (20\%).
%The validation set is utilized for hyperparameter search and calibration. 

\subsubsection{Methods Compared}
%\noindent \textbf{Methods Compared.}
We compare PerK with various traditional and recent methods.
Specifically, we adopt
\begin{itemize}
    \item \textbf{Oracle}: It uses the ground-truth labels of the test set to determine the optimal recommendation size for each user.
\end{itemize}
and three traditional methods:
\begin{itemize}
    \item \textbf{Top-$k$}: It denotes the top-$k$ recommendation with globally fixed recommendation size. We adopt $k \in \{ 1, 5, 10, 20, 50\}$.
    \item \textbf{Rand}: It randomly selects the recommendation size for each user. It represents the lower bound of the performance.
    \item \textbf{Val-$k$}: It selects the recommendation size that maximizes validation utility for each user.
\end{itemize}
and two state-of-the-art methods for truncating document retrieval results:
\begin{itemize}
    \item \textbf{AttnCut} \cite{attncut21}: It deploys a classification model with Bi-LSTM and Transformer encoder to predict the best cut-off position.
    \item \textbf{MtCut} (MMoECut) \cite{mmoecut22}: It deploys MMoE \cite{mmoe18} on top of AttnCut architecture and adopt multi-task learning.
\end{itemize}
and the proposed framework:
\begin{itemize}
    \item \textbf{PerK (ours)}: We determine the personalized recommendation size by estimating the expected user utility with calibrated interaction probability.
\end{itemize}
For a quantitative comparison of user utility, we set the maximum recommendation size to 50 for all methods.
We also tried 100 and observed a similar performance improvement for PerK.

\subsubsection{Base Recommender Models ($f_{\theta}$)}
%\noindent \textbf{Base Recommender Models ($f_{\theta}$).}
% We validate PerK with three widely-used recommender models with various model architectures and loss functions: Bayesian Personalized Ranking (BPR) \cite{bpr09}, Neural Collaborative Filtering (NCF) \cite{ncf17}, and LightGCN \cite{lightgcn20}.
We adopt three widely-used recommender models with various model architectures and loss functions: BPR \cite{bpr09}, NCF \cite{ncf17}, and LightGCN \cite{lightgcn20}.
The ranking score from the base recommender model serves as input for PerK, AttnCut, and MtCut.
%We tune the hyperparameters of the base models by grid search on the validation set.

\input{6EXztable.tex}

\subsection{Comparison of User Utility}
Table 1 presents the average user utility yielded by the recommendation of each compared method.
%In this paper, we adopt four widely-adopted utilities, including NDCG, PDCG, F1, and TP, to quantitatively measure user satisfaction.
%\textit{For all methods, we report the performance when they are optimized for each target utility measure.}
\textit{For a fair comparison, we adopt the same base model and the same target utility throughout the training of AttnCut, MtCut, and PerK in each experimental configuration.}
We report the average result of three independent runs. % For methods with randomness (i.e., Rand, AttnCut, and MtCut), we

% 1. Top-Per-K > Top-K (task)
\noindent \textbf{Benefits of Top-Personalized-$K$ Recommendation.}
We first observe that personalizing the recommendation size results in higher user utility than the globally fixed size.
Oracle shows significantly higher utility compared to the best value of Top-$k$.
This upper bound on user utility highlights the importance of the proposed task in improving user satisfaction.
Accordingly, methods determining the personalized recommendation sizes (i.e., AttnCut, MtCut, and PerK) generally outperform Top-$k$.
Furthermore, we notice that Top-$k$ shows a large performance deviation depending on the recommended size. % and the best global $k$ differs for each utility and dataset.
Therefore, the system should avoid naively setting a globally fixed recommendation size and instead determine the personalized size for improved user satisfaction.

% 2. PerK > other methods for Top-Per-K
\noindent \textbf{Effectiveness of PerK.}
%The proposed PerK outperforms the competitors in the top-personalized-$K$ recommendation task.
We observe that PerK outperforms the competitors in the top-personalized-$K$ recommendation task.
Val-$k$ does not perform well since overfitting to the validation utility is not effective due to the sparse and noisy interactions.
%Furthermore, while the methods for document list truncation (i.e., AttnCut and MtCut) bring slight improvement compared to Top-$k$, their effectiveness remains still limited.
%As discussed in Section 2, the target label for the classification does not provide enough supervision and the scalar ranking scores are not enough for training the large transformer.
%Indeed, we discovered that they can be easily overfitted to select the size that works well globally (Figure 2), resulting in comparable performance to the best of Top-$k$.
%In contrast, PerK does not rely on a deep model and considers the hidden-relevant items, to estimate the expected user utility.
%PerK directly computes the expected user utility in mathematical form with the calibrated interaction probability and significantly outperforms AttnCut and MtCut in the top-personalized-$K$ task.
Furthermore, the effectiveness of the methods for document list truncation (i.e., AttnCut and MtCut) remains limited, since the target label for the classification does not provide enough supervision due to the hidden-positive and noisy interactions.
Indeed, we discovered that they can be easily overfitted to select the size that works well globally (Figure 2), resulting in comparable performance to the best of Top-$k$.
In contrast, PerK does not rely on a deep model and considers the hidden-relevant items, to estimate the expected user utility.
PerK directly computes the expected user utility in mathematical form with the calibrated interaction probability and significantly outperforms AttnCut and MtCut in the top-personalized-$K$ task.

\subsection{Personalized Recommendation Size}
Figure 2 shows the distributions of recommendation sizes determined by Oracle, PerK, and MtCut. % on MovieLens 25M and Amazon Books datasets
The base model is BPR and the target user utility is F1.
We have the following findings:
(1) The distributions of Oracle show that the optimal recommendation size for maximum user utility differs for each user.
(2) The distributions of MtCut are severely skewed towards $k \in [10, 20]$ and have a high peak in that range.
The reason is that MtCut is overfitted to select the globally well-performing $k$ which falls into the range of [10, 20] (refer to F1 on MovieLens 25M and Amazon Books with BPR in Table 1).
(3) The distributions of PerK are smooth and fairly close to those of Oracle.
It is noted that we can set the constraints for the minimum recommendation size in Eq.3, if the system requires it.

% for Sec 6.3
\begin{figure}[t]
\centering 
\begin{subfigure}{0.38\linewidth}
    \includegraphics[width=1\linewidth]{figure/oracle_f1_ml.png}
\end{subfigure}
\vspace{-0.15cm}
\begin{subfigure}{0.295\linewidth}
    \includegraphics[width=1\linewidth]{figure/perk_f1_no_ml.png}
\end{subfigure}
\vspace{-0.15cm}
\begin{subfigure}{0.295\linewidth}
    \includegraphics[width=1\linewidth]{figure/mmoe_f1_no_ml.png}
\end{subfigure}
\vspace{-0.15cm}
\caption*{(a) MovieLens 25M}

\begin{subfigure}{0.38\linewidth}
    \includegraphics[width=1\linewidth]{figure/oracle_f1.png}
\end{subfigure}
\vspace{-0.15cm}
\begin{subfigure}{0.295\linewidth}
    \includegraphics[width=1\linewidth]{figure/perk_f1_no.png}
\end{subfigure}
\vspace{-0.15cm}
\begin{subfigure}{0.295\linewidth}
    \includegraphics[width=1\linewidth]{figure/mmoe_f1_no.png}
\end{subfigure}
\vspace{-0.15cm}
\caption*{(b) Amazon Books}
\vspace{-0.15cm}
\caption{Distribution of recommendation sizes from each method. Three figures in the same row share the y-axis.}
\end{figure}

%% table for NCF
\begin{table}[t]
\caption{Calibration error and user utility for each calibration method. User utilities are computed when each calibration method is applied to PerK. Lower is better for ECE.}
\resizebox{\linewidth}{!}{% 
\begin{tabular}{ccccccc}
\toprule
Dataset & Calibration & ECE $\downarrow$  & NDCG   &PDCG & F1  &TP   \\
\toprule
\multirow{3}{*}{ML10M}  & uncalibrated & 0.1284 & 0.4083 & -0.1071 & 0.1966 & 0.4481\\
    & global            &  0.0046 & 0.4255 & 0.0838 & 0.2175 & 0.4925\\
    & user-wise         &  \textbf{0.0011} & \textbf{0.4482}& \textbf{0.0928} &\textbf{0.2293}  &\textbf{0.5335} \\
\midrule
\multirow{3}{*}{CiteULike}  & uncalibrated & 0.0480 & 0.1811 & -0.5667 & 0.0975 & 0.2512\\
                            & global  & 0.0017 & 0.1940 &-0.5306 & 0.1054 & 0.2639 \\
                            & user-wise & \textbf{0.0003} & \textbf{0.2061}&  \textbf{-0.5177}& \textbf{0.1080} & \textbf{0.2764}\\
\midrule
\multirow{3}{*}{ML25M}      & uncalibrated  & 0.1572 & 0.3612 & -0.2311 & 0.1669 & 0.3812\\
                            & global  & 0.0422 & 0.3761 & -0.1015 & 0.1757 & 0.4007 \\
                            & user-wise & \textbf{0.0098} & \textbf{0.4056}&  \textbf{0.0047}& \textbf{0.1960} & \textbf{0.4742}\\
\midrule
\multirow{3}{*}{ABooks}     & uncalibrated & 0.3371  & 0.0812 & -0.8864 & 0.0427 & 0.1391 \\
                            & global & 0.0581 & 0.0946 & -0.8655 & 0.0449 & 0.1477 \\
                            & user-wise & \textbf{0.0171} & \textbf{0.0982}& \textbf{-0.8646} & \textbf{0.0468} & \textbf{0.1553}\\   
\bottomrule
\end{tabular}}
\setlength{\abovecaptionskip}{-20pt}
\vspace{-0.5cm}
\end{table}

\subsection{Ablation Study for Calibration}
%% table for BPR
\begin{comment}
 \begin{table}[t]
\caption{Calibration error and user utility for each calibration method. The user utility is computed when each calibration method is applied to PerK. Lower is better for ECE.}
\resizebox{\linewidth}{!}{% 
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{l}{Dataset} & \begin{tabular}[c]{@{}c@{}}Calibration\\ method\end{tabular} & ECE$\downarrow$    & NDCG   &PDCG & F1  &TP   \\
\toprule
\multirow{2}{*}{ML10M}      & global                             &  0.0045 & 0.4680 & 0.0479 &0.2441  & 0.5172\\
                            & user-wise                          &  \textbf{0.0018} & \textbf{0.4901}& \textbf{0.2087} &\textbf{0.2538}  &\textbf{0.5711} \\
\midrule
\multirow{2}{*}{CiteULike}      & global                             &0.0062 & 0.2137& -0.5733 & 0.1080 & 0.2873 \\
                            & user-wise                             & \textbf{0.0031} & \textbf{0.2159}&  \textbf{-0.4971}& \textbf{0.1117} & \textbf{0.2993}\\
\midrule
\multirow{2}{*}{ML25M}      & global                                & 0.0433 & 0.4392& 0.0242 & 0.1983 & 0.4972 \\
                            & user-wise                          & \textbf{0.0165} & \textbf{0.4687}&  \textbf{0.1876}& \textbf{0.2300} & \textbf{0.5401}\\
\midrule
\multirow{2}{*}{ABooks}     & global                              & 0.0261 & 0.1076& -0.9947 & 0.0566 & 0.1436 \\
                            & user-wise                          & \textbf{0.0072} & \textbf{0.1261}& \textbf{-0.7952} & \textbf{0.0619} & \textbf{0.1894}\\   
\bottomrule
\end{tabular}}
\end{table}   
\end{comment}

Table 2 presents the ablation study on the calibration method with NCF \cite{ncf17} as a base model. %conducted on four datasets 
We compare (1) the calibration performance, and (2) user utility when it is applied to PerK.% To demonstrate the superiority of the proposed user-wise calibration over the global calibration, 
The calibration performance is measured by Expected Calibration Error (ECE) \cite{bbq15}, a widely used metric for measuring the gap between the output probability and true likelihood of interaction \cite{kweon22, cal17}.
We observe that the proposed user-wise calibration function shows lower ECE than the global calibration function.
Accordingly, PerK yields higher user utilities when it adopts user-wise calibration, demonstrating the superiority of the proposed user-wise calibration over the global calibration.
%indicating that the proposed calibration function is effective in obtaining accurate interaction probability.

\subsection{Space and Time analysis}
\begin{table}[t]
\caption{Space and Time analysis. \#Params. denotes the number of learnable parameters and Time denotes the wall time (in ms) used for generating a ranking list for a user.}
\resizebox{\linewidth}{!}{% 
\begin{tabular}{c|c|cc|cc|cc|cc}
\toprule
Base & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{\textbf{ML10M}} & \multicolumn{2}{c|}{\textbf{CiteULike}} & \multicolumn{2}{c|}{\textbf{ML25M}} & \multicolumn{2}{c}{\textbf{ABooks}} \\
model &                         & \#Params.           & Time            & \#Params.           & Time             & \#Params.           & Time            & \#Params.           & Time           \\
\toprule
\multirow{2}{*}{BPR}        & Top-k                   & 5.041M             & 2.871           & 1.291M              & 2.086            & 11.574M            & 2.374           & 34.542M            & 2.636          \\
                            & PerK                    & 5.181M             & 3.022           & 1.292M              & 2.241            & 11.898M            & 2.652           & 34.857M            & 2.973          \\
\midrule
\multirow{2}{*}{NCF}      & Top-k                   & 10.092M            & 4.092           & 2.581M              & 2.566            & 23.156M            & 3.067           & 69.117M            & 7.767          \\
                            & PerK                    & 10.232M            & 4.406           & 2.588M              & 2.817            & 23.480M            & 3.378           & 69.432M            & 8.871          \\
\midrule
\multirow{2}{*}{LightGCN}       & Top-k                   & 5.042M             & 3.195           & 2.571M              & 2.493            & 23.147M            & 2.628           & 34.542M            & 3.781          \\
                            & PerK                    & 5.181M             & 3.449           & 2.577M              & 2.759            & 23.472M            & 2.969           & 34,857M            & 4.106       \\  
\bottomrule
\end{tabular}}
\setlength{\abovecaptionskip}{-20pt}
\end{table}

\begin{figure}[t]
\centering
    \begin{minipage}[r]{0.49\linewidth}
        \centering
        \begin{subfigure}{0.49\textwidth}
          \includegraphics[width=1\textwidth]{figure/BPR_ML25_NDCG.png}
        \end{subfigure}
        \hspace{-0.1cm}
        \begin{subfigure}{0.5\textwidth}
          \includegraphics[width=1\textwidth]{figure/BPR_ABook_NDCG.png}
        \end{subfigure}
        \hspace{-0.1cm}
        \subcaption{NDCG}
    \end{minipage}
    \hfill%
    \hspace{-0.3cm}
    \begin{minipage}[r]{0.49\linewidth}
        \centering
        \begin{subfigure}{0.5\textwidth}
          \includegraphics[width=1\textwidth]{figure/BPR_ML25_F1.png}
        \end{subfigure}
        \hspace{-0.1cm}
        \begin{subfigure}{0.49\textwidth}
          \includegraphics[width=1\textwidth]{figure/BPR_ABook_F1.png}
        \end{subfigure}
        \subcaption{F1}
    \end{minipage}
    \caption{Hyperparameter study of $M$}
    \setlength{\belowcaptionskip}{-20pt}
    \setlength{\abovecaptionskip}{-5pt}

    \vspace{-0.4cm}
\end{figure}

Table 3 shows the number of learnable parameters and inference time of Top-$k$ and PerK.
The target user utility is NDCG for PerK.
We use PyTorch \cite{pytorch19} with CUDA on GTX Titan Xp GPU and Intel Xeon(R) E5-2640 v4 CPU.
First, PerK does not significantly increase the number of learnable parameters from Top-$k$.
PerK only has two additional parameters for each user for calibration, and it has a negligible impact considering the size of the user embedding is typically selected in the range of 64-128.
Second, the inference time is increased by about 10\%.
To speed up the estimation of expected user utility,
%(1) We perform the user-wise calibration for all users together with a few matrix operations, 
%(2) We estimate the expected user utility with various $k$ in a parallel way,
(1) We perform the user-wise calibration for all users and estimation of the expected user utility with various $k$ in a parallel way,
and (2) We adopt two approximation techniques for fast computation of the expected user utility in Eq.7d.
The hyperparameter study for $M$, which is used for this approximation, with BPR is presented in Figure 3.
We can see that it is enough to aggregate the summation in Eq.7d just to $M=2000$ rather than to the number of all unobserved items $|\mathcal{I}_u^{-}|$. 

%\subsection{Real-world Application Scenarios}
\subsection{Case Study}
\begin{figure}[t]
\centering 
\begin{subfigure}{0.99\linewidth}
    \includegraphics[width=1\linewidth]{figure/casestudy_single.png}
\end{subfigure}
\vspace{-0.3cm}
\caption*{(a) Single-domain scenario on Amazon Books}

\vspace{0.2cm}

\begin{subfigure}{0.99\linewidth}
    \includegraphics[width=1\linewidth]{figure/casestudy-2.png}
\end{subfigure}
\vspace{-0.3cm}
\caption*{(b) Multi-domain scenario on Amazon}
\vspace{-0.3cm}
\caption{Case study. 1 and 0 represent the relevant and the irrelevant labels, which are unavailable at the inference phase. Decimal numbers indicate the F1 score.}

\vspace{-0.5cm}
\end{figure}
%\vspace{-0.5cm}

We present a case study on Amazon dataset to provide concrete examples of how PerK can be applied in real-world applications.
%We analyze the change of user utility on (1) single-domain and (2) multi-domain recommendation scenarios.

\noindent \textbf{Single-domain scenario.}
Figure 4 (a) shows a case study of the single-domain scenario on Amazon Books with BPR as a base model.
The systems often display trending items alongside personalized ones, to create a balanced experience that encompasses both popular choices and items that align with individual preferences.
We determine the number of personalized items with PerK to increase F1 by a large margin, and the remaining slots are then populated with trending items.
In this context, the top-personalized-$K$ recommendation allows the system to strike a balance between the exploration-exploitation trade-off by effectively managing the quantity of personalized items.
% In this case, the system can achieve a balance between exploration-exploitation trade-off by adjusting the number of personalized items With top-personalized-$K$ recommendation.

\noindent \textbf{Multi-domain scenario.}
Figure 4 (b) shows a case study of the multi-domain scenario on the four largest Amazon datasets with BPR as a base model.
We generate top-personalized-$K$ recommendations for each domain by slightly modifying Eq.3, to maximize the average F1 across all domains under the constraint that the total recommendation size should not exceed 40.
We can see that the average F1 score increases as we adopt the top-personalized-$K$ recommendation scheme to strike a balance in the recommendation size of each domain.
This example demonstrates that the top-personalized-$K$ recommendation can be adopted to multi-domain systems for displaying the optimized number of items from each domain on a single constrained page.

%The recommendation size of the top-$K$ recommendation is fixed as ten for both users and PerK determines the recommendation size with respect to NDCG.
%For user 75839, PerK recommends additional two relevant items to increase the user utility.
%On the other hand, for user 17138, PerK excludes two irrelevant items in the tail.
